Synthesizing Permissive Winning Strategy Templates for Parity Games

We present a novel method to compute \emph{permissive winning strategies} in two-player games over finite graphs with $ \omega $-regular winning conditions. Given a game graph $G$ and a parity winning condition $\Phi$, we compute a \emph{winning strategy template} $\Psi$ that collects an infinite number of winning strategies for objective $\Phi$ in a concise data structure. We use this new representation of sets of winning strategies to tackle two problems arising from applications of two-player games in the context of cyber-physical system design -- (i) \emph{incremental synthesis}, i.e., adapting strategies to newly arriving, \emph{additional} $\omega$-regular objectives $\Phi'$, and (ii) \emph{fault-tolerant control}, i.e., adapting strategies to the occasional or persistent unavailability of actuators. The main features of our strategy templates -- which we utilize for solving these challenges -- are their easy computability, adaptability, and compositionality. For \emph{incremental synthesis}, we empirically show on a large set of benchmarks that our technique vastly outperforms existing approaches if the number of added specifications increases. While our method is not complete, our prototype implementation returns the full winning region in all 1400 benchmark instances, i.e., handling a large problem class efficiently in practice.

==> sections/conclusion.tex <==
% !TeX root = ../main.tex

\section{Conclusion and Related Works}
We consider the problem of synthesis of winning strategies for conjunctive combination of objectives. Chatterjee et al. \AAn{needCite} prove that the conjunction of even two parity objectives makes the problem NP-complete. They provide a generalization of Zeilonka algorithm for generalized parity objectives (conjunction of parity objectives), which performs well in practice despite the exponential time complexity in the sum of numbers of priorities in each parity objective. Interestingly, Bouyer et al. show that there are instances where the generalized Zeilonka algorithm fails, calling for a further study of the problem. It is natural to decompose the combination into individual objectives \AAn{Citation}. However, these techniques often work when all the objectives are given, and need recomputation when new objectives are added to existing ones. We tackle this problem by considering a huge set of winning strategies defined by templates (combination of safety edges, live groups and co-live edges) for individual objectives and by composing them together to find strategies that satisfy all of them. The idea behind the templates is to allow the system as many behaviors as possible to satisfy the objectives to come, in other words, the templates are \emph{permissive}.  

The notion of permissiveness has been introduced by many previous works\AAn{Cite}for. Bernet et al. \AAn{Igor's paper} introduce permissive strategies that encompasses all the behaviors of positional strategies. Neider et al. \AAn{cite} introduce permissiveness to subsume strategies that visit losing loops at most twice. Bouyer et al. \AAn{cite} take a quantitative approach to measure permissiveness of strategies, by minimizing the penalty of not being permissive. However, all these approaches fail to preserve enough behaviors to be able to satisfy subsequent objectives, making them unfavorable for compositional synthesis. \AAn{Give examples}

Baier et al. \AAn{cite} give the most general controllers for individual objectives, but fail to employ them to combination of objectives without restricting the plays. \AAn{give example}. In their paper, Bouyer et al. combine generalized Zeilonka algorithm with partial solvers for parity games to obtain partial solutions to the generalized parity objectives, i.e. give regions (not necessarily, partitions) $ \wino $ and $ \winl $ such that they are winning for $ \pz $ and $ \po $ respectively. However, we find randomly generated instances where their algorithms give superset of system's winning region, hence compromising soundness. Since the paper lacks rigorous proofs for the algorithms, it is not clear if it an implementation bug or a theoretical mishap. Regardless, their algorithms again lacks scalability in the online scenario. \AAn{Give examples}.

Our implementation testifies that while our approach of using permissive strategy templates for composition is not complete and is not faster in many cases, it is still comparable to the existing algorithms. Moreover, it gives the correct winning region in most cases. Besides that, as we have discussed before, in addition to the winning region and a strategy template, our algorithm also gives an insight which can later be used to analyze the game.


